DiffusedWrinkles: A Diffusion-Based Model for Data-Driven Garment Animation

We present a data-driven method for learning to generate animations of 3D garments using a 2D image diffusion model. In contrast to existing methods, typically based on fully connected networks, graph neural networks, or generative adversarial networks, which have difficulties to cope with parametric garments with fine wrinkle detail, our approach is able to synthesize high-quality 3D animations for a wide variety of garments and body shapes, while being agnostic to the garment mesh topology. Our key idea is to represent 3D garment deformations as a 2D layout-consistent texture that encodes 3D offsets with respect to a parametric garment template. Using this representation, we encode a large dataset of garments simulated in various motions and shapes and train a novel conditional diffusion model that is able to synthesize high-quality pose-shape-and-design dependent 3D garment deformations. Since our model is generative, we can synthesize various plausible deformations for a given target pose, shape, and design. Additionally, we show that we can further condition our model using an existing garment state, which enables the generation of temporally coherent sequences.

==> bmvc_review <==
\begin{thebibliography}{88}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Arjovsky and Bottou(2017)]{arjovsky2017towards}
Martin Arjovsky and Leon Bottou.
\newblock {Towards Principled Methods for Training Generative Adversarial Networks}.
\newblock In \emph{International Conference on Learning Representations}, 2017.
\newblock URL \url{https://openreview.net/forum?id=Hk4_qw5xe}.

\bibitem[Baraff and Witkin(1998)]{Baraff1998}
David Baraff and Andrew Witkin.
\newblock {Large Steps in Cloth Simulation}.
\newblock In \emph{Proc. of Conference on Computer Graphics and Interactive Techniques (SIGGRAPH)}, page 43–54, 1998.
\newblock \doi{10.1145/280814.280821}.

\bibitem[Berthouzoz et~al.(2013)Berthouzoz, Garg, Kaufman, Grinspun, and Agrawala]{berthouzoz2013parsing}
Floraine Berthouzoz, Akash Garg, Danny~M Kaufman, Eitan Grinspun, and Maneesh Agrawala.
\newblock {Parsing Sewing Patterns into 3D Garments}.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH)}, 32\penalty0 (4):\penalty0 1--12, 2013.
\newblock \doi{10.1145/2461912.2461975}.

\bibitem[Bertiche et~al.(2021)Bertiche, Madadi, and Escalera]{bertiche2021pbns}
Hugo Bertiche, Meysam Madadi, and Sergio Escalera.
\newblock {PBNS: Physically Based Neural Simulation for Unsupervised Garment Pose Space Deformation}.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH Asia)}, 40\penalty0 (6), 2021.
\newblock \doi{10.1145/3478513.3480479}.

\bibitem[Blattmann et~al.(2023)Blattmann, Rombach, Ling, Dockhorn, Kim, Fidler, and Kreis]{blattmann2023align}
Andreas Blattmann, Robin Rombach, Huan Ling, Tim Dockhorn, Seung~Wook Kim, Sanja Fidler, and Karsten Kreis.
\newblock Align your latents: High-resolution video synthesis with latent diffusion models.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 22563--22575, 2023.

\bibitem[Bouaziz et~al.(2014)Bouaziz, Martin, Liu, Kavan, and Pauly]{bouaziz2014projective}
Sofien Bouaziz, Sebastian Martin, Tiantian Liu, Ladislav Kavan, and Mark Pauly.
\newblock { Projective Dynamics: Fusing Constraint Projections for Fast Simulation}.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH)}, 33\penalty0 (4):\penalty0 1--11, 2014.
\newblock \doi{10.1145/2601097.2601116}.

\bibitem[Chen et~al.(2023)Chen, Jiang, Liu, Huang, Fu, Chen, and Yu]{chen2023executing}
Xin Chen, Biao Jiang, Wen Liu, Zilong Huang, Bin Fu, Tao Chen, and Gang Yu.
\newblock Executing your commands via motion diffusion in latent space.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 18000--18010, 2023.

\bibitem[Cirio et~al.(2015)Cirio, Lopez-Moreno, and Otaduy]{cirio2015efficient}
Gabriel Cirio, Jorge Lopez-Moreno, and Miguel~A Otaduy.
\newblock Efficient simulation of knitted cloth using persistent contacts.
\newblock In \emph{Proc. of ACM SIGGRAPH / Eurographics Symposium on Computer Animation (SCA)}, pages 55--61, 2015.
\newblock \doi{10.1145/2786784.2786801}.

\bibitem[Corona et~al.(2021)Corona, Pumarola, Aleny{\`a}, Pons-Moll, and Moreno-Noguer]{corona2021smplicit}
Enric Corona, Albert Pumarola, Guillem Aleny{\`a}, Gerard Pons-Moll, and Francesc Moreno-Noguer.
\newblock {SMPLicit: Topology-aware Generative Model for Clothed People}.
\newblock In \emph{Proc. of Computer Vision and Pattern Recognition (CVPR)}, 2021.

\bibitem[Croitoru et~al.(2023)Croitoru, Hondru, Ionescu, and Shah]{croitoru2023diffusion}
Florinel-Alin Croitoru, Vlad Hondru, Radu~Tudor Ionescu, and Mubarak Shah.
\newblock {Diffusion Models in Vision: A survey}.
\newblock \emph{IEEE Transactions on Pattern Analysis and Machine Intelligence}, 2023.
\newblock \doi{10.1109/TPAMI.2023.3261988}.

\bibitem[De~Aguiar et~al.(2010)De~Aguiar, Sigal, Treuille, and Hodgins]{de2010stable}
Edilson De~Aguiar, Leonid Sigal, Adrien Treuille, and Jessica~K Hodgins.
\newblock Stable spaces for real-time clothing.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH)}, 29\penalty0 (4), 2010.
\newblock \doi{10.1145/1778765.1778843}.

\bibitem[Du et~al.(2023)Du, Kips, Pumarola, Starke, Thabet, and Sanakoyeu]{du2023avatars}
Yuming Du, Robin Kips, Albert Pumarola, Sebastian Starke, Ali Thabet, and Artsiom Sanakoyeu.
\newblock Avatars grow legs: Generating smooth human motion from sparse tracking inputs with diffusion model.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 481--490, 2023.

\bibitem[Fulton et~al.(2019)Fulton, Modi, Duvenaud, Levin, and Jacobson]{fulton2019latent}
Lawson Fulton, Vismay Modi, David Duvenaud, David~IW Levin, and Alec Jacobson.
\newblock {Latent-space Dynamics for Reduced Deformable Simulation}.
\newblock \emph{Computer Graphics Forum (Proc. Eurographics)}, 38\penalty0 (2):\penalty0 379--391, 2019.
\newblock \doi{10.1111/cgf.13645}.

\bibitem[Gillette et~al.(2015)Gillette, Peters, Vining, Edwards, and Sheffer]{gillette2015realtime}
Russell Gillette, Craig Peters, Nicholas Vining, Essex Edwards, and Alla Sheffer.
\newblock {Real-Time Dynamic Wrinkling of Coarse Animated Cloth}.
\newblock In \emph{Proc. of ACM SIGGRAPH / Eurographics Symposium on Computer Animation (SCA)}, 2015.
\newblock \doi{10.1145/2786784.2786789}.

\bibitem[Grigorev et~al.(2023)Grigorev, Thomaszewski, Black, and Hilliges]{grigorev2023hood}
Artur Grigorev, Bernhard Thomaszewski, Michael~J Black, and Otmar Hilliges.
\newblock {HOOD}: Hierarchical graphs for generalized modelling of clothing dynamics.
\newblock In \emph{Proc. of Computer Vision and Pattern Recognition (CVPR)}, 2023.

\bibitem[Guan et~al.(2012)Guan, Reiss, Hirshberg, Weiss, and Black]{guan2012drape}
Peng Guan, Loretta Reiss, David~A Hirshberg, Alexander Weiss, and Michael~J Black.
\newblock {DRAPE: DRessing Any PErson}.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH)}, 31\penalty0 (4), 2012.
\newblock \doi{10.1145/2185520.2185531}.

\bibitem[Gundogdu et~al.(2019)Gundogdu, Constantin, Seifoddini, Dang, Salzmann, and Fua]{gundogdu2019garnet}
Erhan Gundogdu, Victor Constantin, Amrollah Seifoddini, Minh Dang, Mathieu Salzmann, and Pascal Fua.
\newblock {GarNet: A two-stream network for fast and accurate 3D cloth draping}.
\newblock In \emph{Proc. of IEEE International Conference on Computer Vision (ICCV)}, 2019.
\newblock \doi{10.1109/ICCV.2019.00883}.

\bibitem[Ho et~al.(2020)Ho, Jain, and Abbeel]{ho2020denoising}
Jonathan Ho, Ajay Jain, and Pieter Abbeel.
\newblock {Denoising Diffusion Probabilistic Models}.
\newblock \emph{Advances in Neural Information Processing Systems (NeurIPS)}, 33:\penalty0 6840--6851, 2020.

\bibitem[Ho et~al.(2022{\natexlab{a}})Ho, Saharia, Chan, Fleet, Norouzi, and Salimans]{hoJMLR22cascade}
Jonathan Ho, Chitwan Saharia, William Chan, David~J. Fleet, Mohammad Norouzi, and Tim Salimans.
\newblock {Cascaded Diffusion Models for High Fidelity Image Generation}.
\newblock \emph{Journal of Machine Learning Research}, 23\penalty0 (47):\penalty0 1--33, 2022{\natexlab{a}}.
\newblock URL \url{http://jmlr.org/papers/v23/21-0635.html}.

\bibitem[Ho et~al.(2022{\natexlab{b}})Ho, Salimans, Gritsenko, Chan, Norouzi, and Fleet]{hovideo}
Jonathan Ho, Tim Salimans, Alexey~A Gritsenko, William Chan, Mohammad Norouzi, and David~J Fleet.
\newblock Video diffusion models.
\newblock In \emph{Advances in Neural Information Processing Systems (NeurIPS)}, 2022{\natexlab{b}}.

\bibitem[Holden et~al.(2019)Holden, Duong, Datta, and Nowrouzezahrai]{holden2019neuralphysics}
Daniel Holden, Bang~Chi Duong, Sayantan Datta, and Derek Nowrouzezahrai.
\newblock {Subspace Neural Physics: Fast Data-Driven Interactive Simulation}.
\newblock In \emph{Proc. of ACM SIGGRAPH / Eurographics Symposium on Computer Animation (SCA)}, 2019.
\newblock \doi{10.1145/3309486.3340245}.

\bibitem[Hong et~al.(2022)Hong, Zhang, Pan, Cai, Yang, and Liu]{hong2022avatarclip}
Fangzhou Hong, Mingyuan Zhang, Liang Pan, Zhongang Cai, Lei Yang, and Ziwei Liu.
\newblock {AvatarCLIP: Zero-Shot Text-Driven Generation and Animation of 3D Avatars}.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH)}, 41\penalty0 (4), 2022.

\bibitem[House and Breen(2000)]{house2000cloth}
Donald House and David Breen.
\newblock \emph{{Cloth Modeling and Animation}}.
\newblock CRC Press, 2000.

\bibitem[Hu et~al.(2020)Hu, Anderson, Li, Sun, Carr, Ragan-Kelley, and Durand]{hu2020difftaichi}
Yuanming Hu, Luke Anderson, Tzu-Mao Li, Qi~Sun, Nathan Carr, Jonathan Ragan-Kelley, and Fr{\'e}do Durand.
\newblock {DiffTaichi: Differentiable Programming for Physical Simulation}.
\newblock In \emph{International Conference on Learning Representations}, 2020.

\bibitem[Jiang et~al.(2022)Jiang, Yang, Qiu, Wu, Loy, and Liu]{jiang2022text2human}
Yuming Jiang, Shuai Yang, Haonan Qiu, Wayne Wu, Chen~Change Loy, and Ziwei Liu.
\newblock {Text2Human: Text-Driven Controllable Human Image Generation}.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH)}, 41\penalty0 (4), 2022.

\bibitem[Jin et~al.(2020)Jin, Zhu, Geng, and Fedkiw]{jin2020pixel}
Ning Jin, Yilin Zhu, Zhenglin Geng, and Ron Fedkiw.
\newblock {A Pixel-Based Framework for Data-Driven Clothing}.
\newblock \emph{Computer Graphics Forum (Proc. of SCA)}, 2020.
\newblock \doi{10.1111/cgf.14108}.

\bibitem[Joo et~al.(2018)Joo, Simon, and Sheikh]{joo2018total}
Hanbyul Joo, Tomas Simon, and Yaser Sheikh.
\newblock {Total Capture: A 3D Deformation Model for Tracking Faces, Hands, and Bodies}.
\newblock In \emph{Proc. of Computer Vision and Pattern Recognition (CVPR)}, 2018.

\bibitem[Kaldor et~al.(2010)Kaldor, James, and Marschner]{kaldor2010efficient}
Jonathan~M Kaldor, Doug~L James, and Steve Marschner.
\newblock Efficient yarn-based cloth with adaptive contact linearization.
\newblock In \emph{Proc of ACM SIGGRAPH}, 2010.
\newblock \doi{10.1145/1833349.1778842}.

\bibitem[Kavan et~al.(2011)Kavan, Gerszewski, Bargteil, and Sloan]{kavan2011physics}
Ladislav Kavan, Dan Gerszewski, Adam~W Bargteil, and Peter-Pike Sloan.
\newblock Physics-inspired upsampling for cloth simulation in games.
\newblock In \emph{ACM SIGGRAPH 2011 papers}, pages 1--10. ACM, 2011.

\bibitem[Kim et~al.(2022)Kim, Kim, and Choi]{kim2022flame}
Jihoon Kim, Jiseob Kim, and Sungjoon Choi.
\newblock Flame: Free-form language-based motion synthesis \& editing.
\newblock \emph{arXiv preprint arXiv:2209.00349}, 2022.

\bibitem[Kim et~al.(2012)Kim, Chentanez, and M{\"u}ller-Fischer]{kim2012long}
Tae-Yong Kim, Nuttapong Chentanez, and Matthias M{\"u}ller-Fischer.
\newblock {Long range attachments -- A method to simulate inextensible clothing in computer games}.
\newblock In \emph{Proc. of ACM SIGGRAPH / Eurographics Symposium on Computer Animation (SCA)}, pages 305--310, 2012.
\newblock \doi{10.5555/2422356.2422399}.

\bibitem[Kolotouros et~al.(2023)Kolotouros, Alldieck, Zanfir, Bazavan, Fieraru, and Sminchisescu]{kolotouros2023dreamhuman}
Nikos Kolotouros, Thiemo Alldieck, Andrei Zanfir, Eduard~Gabriel Bazavan, Mihai Fieraru, and Cristian Sminchisescu.
\newblock {DreamHuman: Animatable 3D Avatars from Text}.
\newblock \emph{arXiv preprint arXiv:2306.09329}, 2023.

\bibitem[Korosteleva and Lee(2022)]{korosteleva2022neuraltailor}
Maria Korosteleva and Sung-Hee Lee.
\newblock {NeuralTailor: Reconstructing Sewing Pattern Structures from 3D Point Clouds of Garments}.
\newblock \emph{ACM Trans. Graph.}, 41\penalty0 (4), 2022.
\newblock \doi{10.1145/3528223.3530179}.

\bibitem[L\"ahner et~al.(2018)L\"ahner, Cremers, and Tung]{lahner2018deepwrinkles}
Zorah L\"ahner, Daniel Cremers, and Tony Tung.
\newblock {DeepWrinkles: Accurate and Realistic Clothing Modeling}.
\newblock In \emph{Proc. of European Conference on Computer Vision (ECCV)}, 2018.
\newblock \doi{10.1007/978-3-030-01225-0_41}.

\bibitem[Larsen et~al.(2016)Larsen, S\o{}nderby, Larochelle, and Winther]{larsen2016vaegan}
Anders Boesen~Lindbo Larsen, S\o{}ren~Kaae S\o{}nderby, Hugo Larochelle, and Ole Winther.
\newblock {Autoencoding beyond Pixels Using a Learned Similarity Metric}.
\newblock In \emph{Proc. of International Conference on International Conference on Machine Learning (ICML)}, pages 1558--1566, 2016.

\bibitem[Liang et~al.(2019)Liang, Lin, and Koltun]{liang2019differentiable}
Junbang Liang, Ming Lin, and Vladlen Koltun.
\newblock {Differentiable Cloth Simulation for Inverse Problems}.
\newblock In \emph{Advances in Neural Information Processing Systems (NeurIPS)}, pages 771--780, 2019.

\bibitem[Loper et~al.(2015)Loper, Mahmood, Romero, Pons-Moll, and Black]{loper2015smpl}
Matthew Loper, Naureen Mahmood, Javier Romero, Gerard Pons-Moll, and Michael~J Black.
\newblock Smpl: A skinned multi-person linear model.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH Asia)}, 34\penalty0 (6):\penalty0 1--16, 2015.
\newblock \doi{10.1145/2816795.2818013}.

\bibitem[Luo and Hu(2021)]{luo2021diffusion}
Shitong Luo and Wei Hu.
\newblock {Diffusion Probabilistic Models for 3D Point Cloud Generation}.
\newblock In \emph{Proc. of Computer Vision and Pattern Recognition (CVPR)}, pages 2837--2845, 2021.

\bibitem[Luo et~al.(2023)Luo, Chen, Zhang, Huang, Wang, Shen, Zhao, Zhou, and Tan]{luo2023videofusion}
Zhengxiong Luo, Dayou Chen, Yingya Zhang, Yan Huang, Liang Wang, Yujun Shen, Deli Zhao, Jingren Zhou, and Tieniu Tan.
\newblock Videofusion: Decomposed diffusion models for high-quality video generation.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 10209--10218, 2023.

\bibitem[Ma et~al.(2020)Ma, Yang, Ranjan, Pujades, Pons-Moll, Tang, and Black]{ma2020learning}
Qianli Ma, Jinlong Yang, Anurag Ranjan, Sergi Pujades, Gerard Pons-Moll, Siyu Tang, and Michael~J Black.
\newblock Learning to dress 3d people in generative clothing.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 6469--6478, 2020.

\bibitem[Ma et~al.(2021{\natexlab{a}})Ma, Saito, Yang, Tang, and Black]{maCVPR2021}
Qianli Ma, Shunsuke Saito, Jinlong Yang, Siyu Tang, and Michael~J. Black.
\newblock {SCALE: Modeling Clothed Humans with a Surface Codec of Articulated Local Elements}.
\newblock In \emph{Proc. of Computer Vision and Pattern Recognition (CVPR)}, pages 16082--16093, 2021{\natexlab{a}}.

\bibitem[Ma et~al.(2021{\natexlab{b}})Ma, Yang, Tang, and Black]{ma2021pop}
Qianli Ma, Jinlong Yang, Siyu Tang, and Michael~J. Black.
\newblock {The Power of Points for Modeling Humans in Clothing}.
\newblock In \emph{Proc. of IEEE International Conference on Computer Vision (ICCV)}, pages 10974--10984, 2021{\natexlab{b}}.

\bibitem[Mahmood et~al.(2019)Mahmood, Ghorbani, Troje, Pons-Moll, and Black]{AMASS:ICCV:2019}
Naureen Mahmood, Nima Ghorbani, Nikolaus~F. Troje, Gerard Pons-Moll, and Michael~J. Black.
\newblock {AMASS: Archive of Motion Capture as Surface Shapes}.
\newblock In \emph{Proc. of IEEE International Conference on Computer Vision (ICCV)}, pages 5442--5451, October 2019.

\bibitem[Meng et~al.(2023)Meng, Rombach, Gao, Kingma, Ermon, Ho, and Salimans]{meng2023distillation}
Chenlin Meng, Robin Rombach, Ruiqi Gao, Diederik Kingma, Stefano Ermon, Jonathan Ho, and Tim Salimans.
\newblock {On Distillation of Guided Diffusion Models}.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 14297--14306, 2023.

\bibitem[M\"uller et~al.(2007)M\"uller, Heidelberger, Hennix, and Ratcliff]{mueller2007pbd}
Matthias M\"uller, Bruno Heidelberger, Marcus Hennix, and John Ratcliff.
\newblock {Position Based Dynamics}.
\newblock \emph{Journal of Visual Communication and Image Representation}, 18\penalty0 (2), 2007.
\newblock \doi{10.1016/j.jvcir.2007.01.005}.

\bibitem[M{\"u}ller et~al.(2014)M{\"u}ller, Chentanez, Kim, and Macklin]{muller2014strain}
Matthias M{\"u}ller, Nuttapong Chentanez, Tae-Yong Kim, and Miles Macklin.
\newblock {Strain Based Dynamics}.
\newblock In \emph{Proc. of ACM SIGGRAPH / Eurographics Symposium on Computer Animation (SCA)}, pages 149--157, 2014.
\newblock \doi{10.1145/2343483.2343501}.

\bibitem[Narain et~al.(2012)Narain, Samii, and O'brien]{narain2012arcsim}
Rahul Narain, Armin Samii, and James~F O'brien.
\newblock {Adaptive Anisotropic Remeshing for Cloth Simulation}.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH Asia)}, 31\penalty0 (6):\penalty0 1--10, 2012.
\newblock \doi{10.1145/2366145.2366171}.

\bibitem[Nealen et~al.(2006)Nealen, M{\"u}ller, Keiser, Boxerman, and Carlson]{nealen2006physically}
Andrew Nealen, Matthias M{\"u}ller, Richard Keiser, Eddy Boxerman, and Mark Carlson.
\newblock {Physically Based Deformable Models in Computer Graphics}.
\newblock \emph{Computer Graphics Forum}, 25\penalty0 (4):\penalty0 809--836, 2006.

\bibitem[Ni et~al.(2023)Ni, Shi, Li, Huang, and Min]{ni2023conditional}
Haomiao Ni, Changhao Shi, Kai Li, Sharon~X Huang, and Martin~Renqiang Min.
\newblock Conditional image-to-video generation with latent flow diffusion models.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 18444--18455, 2023.

\bibitem[Overby et~al.(2017)Overby, Brown, Li, and Narain]{overby2017admm}
Matthew Overby, George~E Brown, Jie Li, and Rahul Narain.
\newblock {ADMM $\supseteq$ projective dynamics: Fast simulation of hyperelastic models with dynamic constraints}.
\newblock \emph{IEEE Transactions on Visualization and Computer Graphics}, 23\penalty0 (10):\penalty0 2222--2234, 2017.
\newblock \doi{10.1109/TVCG.2017.2730875}.

\bibitem[Patel et~al.(2020)Patel, Liao, and Pons-Moll]{patel2020tailor}
Chaitanya Patel, Zhouyingcheng Liao, and Gerard Pons-Moll.
\newblock {The Virtual Tailor: Predicting Clothing in 3D as a Function of Human Pose, Shape and Garment Style}.
\newblock In \emph{Proc. of Computer Vision and Pattern Recognition (CVPR)}, 2020.

\bibitem[Poole et~al.(2022)Poole, Jain, Barron, and Mildenhall]{poole2022dreamfusion}
Ben Poole, Ajay Jain, Jonathan~T Barron, and Ben Mildenhall.
\newblock Dreamfusion: Text-to-3d using 2d diffusion.
\newblock \emph{arXiv preprint arXiv:2209.14988}, 2022.

\bibitem[Provot et~al.(1995)]{provot1995deformation}
Xavier Provot et~al.
\newblock Deformation constraints in a mass-spring model to describe rigid cloth behaviour.
\newblock In \emph{Graphics interface}, pages 147--147. Canadian Information Processing Society, 1995.

\bibitem[Ramesh et~al.(2022)Ramesh, Dhariwal, Nichol, Chu, and Chen]{ramesh2022hierarchical}
Aditya Ramesh, Prafulla Dhariwal, Alex Nichol, Casey Chu, and Mark Chen.
\newblock Hierarchical text-conditional image generation with clip latents.
\newblock \emph{arXiv preprint arXiv:2204.06125}, 2022.

\bibitem[Ranjan et~al.(2018)Ranjan, Bolkart, Sanyal, and Black]{ranjan2018generating}
Anurag Ranjan, Timo Bolkart, Soubhik Sanyal, and Michael~J Black.
\newblock {Generating 3D Faces Using Convolutional Mesh Autoencoders}.
\newblock In \emph{Proc. of European Conference on Computer Vision (ECCV)}, pages 725--741, 2018.
\newblock \doi{10.1007/978-3-030-01219-9_43}.

\bibitem[Saharia et~al.(2022{\natexlab{a}})Saharia, Chan, Chang, Lee, Ho, Salimans, Fleet, and Norouzi]{saharia2022palette}
Chitwan Saharia, William Chan, Huiwen Chang, Chris Lee, Jonathan Ho, Tim Salimans, David Fleet, and Mohammad Norouzi.
\newblock Palette: Image-to-image diffusion models.
\newblock In \emph{ACM SIGGRAPH 2022 Conference Proceedings}, pages 1--10, 2022{\natexlab{a}}.

\bibitem[Saharia et~al.(2022{\natexlab{b}})Saharia, Chan, Saxena, Li, Whang, Denton, Ghasemipour, Gontijo~Lopes, Karagol~Ayan, Salimans, et~al.]{saharia2022photorealistic}
Chitwan Saharia, William Chan, Saurabh Saxena, Lala Li, Jay Whang, Emily~L Denton, Kamyar Ghasemipour, Raphael Gontijo~Lopes, Burcu Karagol~Ayan, Tim Salimans, et~al.
\newblock Photorealistic text-to-image diffusion models with deep language understanding.
\newblock \emph{Advances in Neural Information Processing Systems}, 35:\penalty0 36479--36494, 2022{\natexlab{b}}.

\bibitem[Santesteban et~al.(2019)Santesteban, Otaduy, and Casas]{santesteban2019virtualtryon}
Igor Santesteban, Miguel~A. Otaduy, and Dan Casas.
\newblock {Learning-Based Animation of Clothing for Virtual Try-On}.
\newblock \emph{Computer Graphics Forum (Proc. Eurographics)}, 38\penalty0 (2), 2019.
\newblock ISSN 1467--8659.
\newblock \doi{10.1111/cgf.13643}.

\bibitem[Santesteban et~al.(2021)Santesteban, Thuerey, Otaduy, and Casas]{santesteban2021garmentcollisions}
Igor Santesteban, Nils Thuerey, Miguel~A Otaduy, and Dan Casas.
\newblock {Self-Supervised Collision Handling via Generative 3D Garment Models for Virtual Try-On}.
\newblock In \emph{Proc. of Computer Vision and Pattern Recognition (CVPR)}, 2021.

\bibitem[Santesteban et~al.(2022)Santesteban, Otaduy, and Casas]{santesteban2022snug}
Igor Santesteban, Miguel~A Otaduy, and Dan Casas.
\newblock {SNUG: Self-supervised Neural Dynamic Garments}.
\newblock In \emph{Proc. of Computer Vision and Pattern Recognition (CVPR)}, pages 8140--8150, 2022.

\bibitem[Sauer et~al.(2023)Sauer, Lorenz, Blattmann, and Rombach]{sauer2023adversarial}
Axel Sauer, Dominik Lorenz, Andreas Blattmann, and Robin Rombach.
\newblock {Adversarial Diffusion Distillation}, 2023.

\bibitem[Selle et~al.(2009)Selle, Su, Irving, and Fedkiw]{selle2008robust}
Andrew Selle, Jonathan Su, Geoffrey Irving, and Ronald Fedkiw.
\newblock {Robust High-Resolution Cloth Using Parallelism, History-Based Collisions, and Accurate Friction}.
\newblock \emph{IEEE Transactions on Visualization and Computer Graphics (TVCG)}, 15\penalty0 (2):\penalty0 339–350, 2009.
\newblock \doi{10.1109/TVCG.2008.79}.

\bibitem[Shen et~al.(2020)Shen, Liang, and Lin]{shen2020gan}
Yu~Shen, Junbang Liang, and Ming~C Lin.
\newblock Gan-based garment generation using sewing pattern images.
\newblock In \emph{European Conference on Computer Vision}, pages 225--247. Springer, 2020.

\bibitem[Sifakis and Barbic(2012)]{sifakis2012fem}
Eftychios Sifakis and Jernej Barbic.
\newblock {FEM simulation of 3D deformable solids: a practitioner's guide to theory, discretization and model reduction}.
\newblock In \emph{SIGGRAPH 2012 Courses}, pages 1--50. ACM, 2012.
\newblock \doi{10.1145/2343483.2343501}.

\bibitem[Singer et~al.(2023)Singer, Polyak, Hayes, Yin, An, Zhang, Hu, Yang, Ashual, Gafni, Parikh, Gupta, and Taigman]{singer2023makeavideo}
Uriel Singer, Adam Polyak, Thomas Hayes, Xi~Yin, Jie An, Songyang Zhang, Qiyuan Hu, Harry Yang, Oron Ashual, Oran Gafni, Devi Parikh, Sonal Gupta, and Yaniv Taigman.
\newblock Make-a-video: Text-to-video generation without text-video data.
\newblock In \emph{The Eleventh International Conference on Learning Representations}, 2023.
\newblock URL \url{https://openreview.net/forum?id=nJfylDvgzlq}.

\bibitem[Su et~al.(2023)Su, Yu, Wang, and Liu]{su2022deepcloth}
Zhaoqi Su, Tao Yu, Yangang Wang, and Yebin Liu.
\newblock {DeepCloth: Neural Garment Representation for Shape and Style Editing}.
\newblock \emph{IEEE Transactions on Pattern Analysis and Machine Intelligence}, 45\penalty0 (2):\penalty0 1581--1593, 2023.
\newblock \doi{10.1109/TPAMI.2022.3168569}.

\bibitem[Tang et~al.(2018)Tang, Wang, Liu, Tong, and Manocha]{tang2018gpu}
Min Tang, Tongtong Wang, Zhongyuan Liu, Ruofeng Tong, and Dinesh Manocha.
\newblock {I-Cloth: Incremental Collision Handling for GPU-Based Interactive Cloth Simulation}.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH Asia)}, 37\penalty0 (6), 2018.
\newblock \doi{10.1145/3272127.3275005}.

\bibitem[Tevet et~al.(2022)Tevet, Raab, Gordon, Shafir, Bermano, and Cohen-Or]{tevet2022human}
Guy Tevet, Sigal Raab, Brian Gordon, Yonatan Shafir, Amit~H Bermano, and Daniel Cohen-Or.
\newblock Human motion diffusion model.
\newblock \emph{arXiv preprint arXiv:2209.14916}, 2022.

\bibitem[Tiwari et~al.(2020)Tiwari, Bhatnagar, Tung, and Pons-Moll]{tiwari20sizer}
Garvita Tiwari, Bharat~Lal Bhatnagar, Tony Tung, and Gerard Pons-Moll.
\newblock {SIZER: A Dataset and Model for Parsing 3D Clothing and Learning Size Sensitive 3D Clothing}.
\newblock In \emph{Proc. of European Conference on Computer Vision (ECCV)}, 2020.

\bibitem[Tiwari et~al.(2021)Tiwari, Sarafianos, Tung, and Pons-Moll]{tiwari21neuralgif}
Garvita Tiwari, Nikolaos Sarafianos, Tony Tung, and Gerard Pons-Moll.
\newblock {Neural-GIF: Neural Generalized Implicit Functions for Animating People in Clothing}.
\newblock In \emph{Proc. of IEEE International Conference on Computer Vision (ICCV)}, 2021.

\bibitem[Um et~al.(2020)Um, Brand, Fei, Holl, and Thuerey]{um2020solver}
Kiwon Um, Robert Brand, Yun~Raymond Fei, Philipp Holl, and Nils Thuerey.
\newblock Solver-in-the-loop: Learning from differentiable physics to interact with iterative pde-solvers.
\newblock \emph{Advances in Neural Information Processing Systems}, 33:\penalty0 6111--6122, 2020.

\bibitem[Umetani et~al.(2011)Umetani, Kaufman, Igarashi, and Grinspun]{umetani2011sensitive}
Nobuyuki Umetani, Danny~M. Kaufman, Takeo Igarashi, and Eitan Grinspun.
\newblock Sensitive couture for interactive garment modeling and editing.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH)}, 30\penalty0 (4), 2011.
\newblock \doi{10.1145/2010324.1964985}.

\bibitem[Vaswani et~al.(2017)Vaswani, Shazeer, Parmar, Uszkoreit, Jones, Gomez, Kaiser, and Polosukhin]{vaswani2017attention}
Ashish Vaswani, Noam Shazeer, Niki Parmar, Jakob Uszkoreit, Llion Jones, Aidan~N Gomez, {\L}ukasz Kaiser, and Illia Polosukhin.
\newblock Attention is all you need.
\newblock \emph{Advances in neural information processing systems}, 30, 2017.

\bibitem[Vidaurre et~al.(2020)Vidaurre, Santesteban, Garces, and Casas]{vidaurre2020virtualtryon}
Raquel Vidaurre, Igor Santesteban, Elena Garces, and Dan Casas.
\newblock {Fully Convolutional Graph Neural Networks for Parametric Virtual Try-On}.
\newblock \emph{Computer Graphics Forum (Proc. SCA)}, 39\penalty0 (8), 2020.
\newblock \doi{10.1111/cgf.14109}.

\bibitem[Voleti et~al.(2022)Voleti, Jolicoeur-Martineau, and Pal]{voleti2022MCVD}
Vikram Voleti, Alexia Jolicoeur-Martineau, and Christopher Pal.
\newblock Mcvd: Masked conditional video diffusion for prediction, generation, and interpolation.
\newblock In \emph{(NeurIPS) Advances in Neural Information Processing Systems}, 2022.
\newblock URL \url{https://arxiv.org/abs/2205.09853}.

\bibitem[Wang(2021)]{wang2021gpu}
Huamin Wang.
\newblock {GPU-based simulation of cloth wrinkles at submillimeter levels}.
\newblock \emph{ACM Transactions on Graphics (TOG)}, 40\penalty0 (4):\penalty0 1--14, 2021.
\newblock \doi{10.1145/3450626.3459787}.

\bibitem[Wang et~al.(2019)Wang, Shao, Fu, and Mitra]{wang2019intrisicspace}
Tuanfeng~Y Wang, Tianjia Shao, Kai Fu, and Niloy~J Mitra.
\newblock {Learning an Intrinsic Garment Space for Interactive Authoring of Garment Animation}.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH Asia)}, 38\penalty0 (6), 2019.
\newblock \doi{10.1145/3355089.3356512}.

\bibitem[Wu et~al.(2022)Wu, Wang, and Wang]{wu2022gpu}
Botao Wu, Zhendong Wang, and Huamin Wang.
\newblock {A GPU-Based Multilevel Additive Schwarz Preconditioner for Cloth and Deformable Body Simulation}.
\newblock \emph{ACM Transactions on Graphics (TOG)}, 41\penalty0 (4):\penalty0 1--14, 2022.
\newblock \doi{10.1145/3528223.3530085}.

\bibitem[Xu et~al.(2014)Xu, Umentani, Chao, Mao, Jin, and Tong]{xu2014sensitivity}
Weiwei Xu, Nobuyuki Umentani, Qianwen Chao, Jie Mao, Xiaogang Jin, and Xin Tong.
\newblock Sensitivity-optimized rigging for example-based real-time clothing synthesis.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH)}, 33\penalty0 (4), 2014.
\newblock \doi{10.1145/2601097.2601136}.

\bibitem[Xu et~al.(2019)Xu, Yang, Sun, Tan, Li, and Zhou]{xu20193d}
Yi~Xu, Shanglin Yang, Wei Sun, Li~Tan, Kefeng Li, and Hui Zhou.
\newblock {3D Virtual Garment Modeling from RGB Images}.
\newblock In \emph{IEEE International Symposium on Mixed and Augmented Reality (ISMAR)}, pages 37--45, 2019.
\newblock \doi{10.1109/ISMAR.2019.00-28}.

\bibitem[Yu et~al.(2023)Yu, Sohn, Kim, and Shin]{yu2023video}
Sihyun Yu, Kihyuk Sohn, Subin Kim, and Jinwoo Shin.
\newblock Video probabilistic diffusion models in projected latent space.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 18456--18466, 2023.

\bibitem[Zakharkin et~al.(2021)Zakharkin, Mazur, Grigorev, and Lempitsky]{zakharkin2021ICCV}
Ilya Zakharkin, Kirill Mazur, Artur Grigorev, and Victor Lempitsky.
\newblock {Point-Based Modeling of Human Clothing}.
\newblock In \emph{Proc. of IEEE International Conference on Computer Vision (ICCV)}, 2021.

\bibitem[Zhang et~al.(2023)Zhang, Chen, Yang, Qu, Wang, Chen, Long, Zhu, Du, and Zheng]{zhang2023avatarverse}
Huichao Zhang, Bowen Chen, Hao Yang, Liao Qu, Xu~Wang, Li~Chen, Chao Long, Feida Zhu, Kang Du, and Min Zheng.
\newblock {AvatarVerse: High-quality \& Stable 3D Avatar Creation from Text and Pose}.
\newblock \emph{arXiv preprint arXiv:2308.03610}, 2023.

\bibitem[Zhang et~al.(2021{\natexlab{a}})Zhang, Wang, Ceylan, and Mitra]{zhang2021deep}
Meng Zhang, Tuanfeng Wang, Duygu Ceylan, and Niloy~J Mitra.
\newblock {Deep Detail Enhancement for Any Garment}.
\newblock \emph{Computer Graphics Forum}, 40\penalty0 (2):\penalty0 399--411, 2021{\natexlab{a}}.
\newblock \doi{10.1111/cgf.142642}.

\bibitem[Zhang et~al.(2021{\natexlab{b}})Zhang, Wang, Ceylan, and Mitra]{zhang2021dynamic}
Meng Zhang, Tuanfeng~Y Wang, Duygu Ceylan, and Niloy~J Mitra.
\newblock {Dynamic Neural Garments}.
\newblock \emph{ACM Transactions on Graphics (TOG)}, 40\penalty0 (6):\penalty0 1--15, 2021{\natexlab{b}}.
\newblock \doi{10.1145/3478513.3480497}.

\bibitem[Zhang et~al.(2022{\natexlab{a}})Zhang, Ceylan, and Mitra]{zhang2022motionguided}
Meng Zhang, Duygu Ceylan, and Niloy~J. Mitra.
\newblock {Motion Guided Deep Dynamic 3D Garments}.
\newblock \emph{ACM Transactions on Graphics (Proc. SIGGRAPH Asia)}, 41\penalty0 (6), 2022{\natexlab{a}}.
\newblock \doi{10.1145/3550454.3555485}.

\bibitem[Zhang et~al.(2022{\natexlab{b}})Zhang, Cai, Pan, Hong, Guo, Yang, and Liu]{zhang2022motiondiffuse}
Mingyuan Zhang, Zhongang Cai, Liang Pan, Fangzhou Hong, Xinying Guo, Lei Yang, and Ziwei Liu.
\newblock Motiondiffuse: Text-driven human motion generation with diffusion model.
\newblock \emph{arXiv preprint arXiv:2208.15001}, 2022{\natexlab{b}}.

\bibitem[Zurdo et~al.(2012)Zurdo, Brito, and Otaduy]{zurdo2012animating}
Javier~S Zurdo, Juan~P Brito, and Miguel~A Otaduy.
\newblock {Animating Wrinkles by Example on Non-Skinned Cloth}.
\newblock \emph{IEEE Transactions on Visualization and Computer Graphics (TVCG)}, 19\penalty0 (1):\penalty0 149--158, 2012.
\newblock \doi{10.1109/TVCG.2012.79}.

\end{thebibliography}

